Alternating linear scheme in a Bayesian framework for low-rank tensor approximation

Multiway data often naturally occurs in a tensorial format which can be approximately represented by a low-rank tensor decomposition. This is useful because complexity can be significantly reduced and the treatment of large-scale data sets can be facilitated. In this paper, we find a low-rank representation for a given tensor by solving a Bayesian inference problem. This is achieved by dividing the overall inference problem into sub-problems where we sequentially infer the posterior distribution of one tensor decomposition component at a time. This leads to a probabilistic interpretation of the well-known iterative algorithm alternating linear scheme (ALS). In this way, the consideration of measurement noise is enabled, as well as the incorporation of application-specific prior knowledge and the uncertainty quantification of the low-rank tensor estimate. To compute the low-rank tensor estimate from the posterior distributions of the tensor decomposition components, we present an algorithm that performs the unscented transform in tensor train format.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}

==> parking.tex <==
As mentioned in \cref{sec:intro}, to formulate the linear least squares problem for one update of the ALS, the TD's property of multi-linearity is exploited and it is expressed as $\y = \U_{\setminus n}\g_n$, with $\U_{\setminus n} \in \mathbb{R}^{J \times K}$ and $\g_n\in \mathbb{R}^{K\times 1}$, where $J$ and $K$ are the number of elements of  $\Yt$ and $\Gt_n$, respectively. The following three examples describe how $\U_{\setminus n}$ is built for the CP decomposition, the Tucker decomposition, and the TT decomposition. Suppose we have a three-way tensor $\Yt$ of size $I_1\times I_2\times I_3$ and uniform ranks $R$, and we would like to update the second core.

\begin{example}
If the tensor is represented in terms of a CP decomposition, the matrix $\U_{\setminus n}$ for $n=2$ can be written as
\begin{equation}
    \U_{\setminus 2} = \left(\G_3 \odot \G_1 \right)\otimes \id_{I_2} \in \mathbb{R}^{I_2I_1I_3\times I_2R}
    \label{eq:U_cp}
\end{equation}
\hl{Note that $\U_{\setminus n}$ first dimension is permuted with respect to $\y\in\mathbb{R}^{I_1I_2I_3}$.}
\end{example}
\hl{Generally, the weight vector $\boldsymbol\lambda$ is absorbed into the factor matrix that is being updated. After each update, the columns of $\G_n$ are normalized and the norms are stored in $\boldsymbol\lambda$. The CP-ALS algorithm can be found in} \cite[p.\ 471]{Kolda2009}.
\begin{example}[\textbf{Tucker decomposition}]
If the tensor is represented in terms of a Tucker decomposition, the matrix $\U_{\setminus n}$ for $n=2$ can be written as
\begin{equation}
    \U_{\setminus 2} = \left[\left( \G_3 \otimes \G_1 \right) \mathbf{C}_{(2)}^\top\right]\otimes \id_{I_2} \in \mathbb{R}^{I_2I_1I_3\times I_2R}.
    \label{eq:U_tucker}
\end{equation}
\hl{Note that $\U_{\setminus 2}$ first dimension is permuted with respect to $\y\in\mathbb{R}^{I_1I_2I_3}$.}
\end{example}
\hl{After every update the core tensor is recomputed by solving}
\begin{equation}
    \y = (\G_3\otimes\G_2\otimes\G_1)\operatorname{vec}(\mathbfcal{C}).
\end{equation}
\hl{In case that the Tucker decomposition has orthogonal factor matrices, the updated core is orthogonalized and the Frobenius norm of the updated core is absorbed into the core tensor. For the TT decomposition we consider the general case with a tensor of size~$I_1I_2\dots I_N$.}
\begin{example}
\label{ex:ttd}
If the tensor is represented in terms of a TT decomposition, the matrix $\U_{\setminus n}$ can be written as 
\begin{equation}
\U_{\setminus n} = \Gt_{i>n}\otimes \id_{I_n} \otimes \Gt_{i<n}^\top \in\mathbb{R}^{I_1I_2\dots I_N\times RI_nR},
\label{eq:multilin}
\end{equation}
where $\Gt_{i<n}$ ($\Gt_{i>n}$) denotes a tensor obtained by contracting the TD components, left (right) of the $n$th core.
\end{example}   
